Challenges in Net Neutrality Violation Detection: A Case Study of Wehe Tool and Improvements

We consider the problem of detecting deliberate traffic discrimination on the Internet. Given the complex nature of the Internet, detection of deliberate discrimination is not easy to detect, and tools developed so far suffer from various limitations. We study challenges in detecting the violations (focusing on the HTTPS traffic) and discuss possible mitigation approaches. We focus on `Wehe,' the most recent tool developed to detect net-neutrality violations. Wehe hosts traffic from all services of interest in a common server and replays them to mimic the behavior of the traffic from original servers. Despite Wehe's vast utility and possible influences over policy decisions, its mechanisms are not yet validated by others. In this work, we highlight critical weaknesses in Wehe where its replay traffic is not being correctly classified as intended services by the network middleboxes. We validate this observation using a commercial traffic shaper. We propose a new method in which the SNI parameter is set appropriately in the initial TLS handshake to overcome this weakness. Using commercial traffic shapers, we validate that SNI makes the replay traffic gets correctly classified as the intended traffic by the middleboxes. Our new approach thus provides a more realistic method for detecting neutrality violations of HTTPS traffic.

==> sum_find.tex <==
The Wehe tool validation results have surfaced its noncompliance to TD detection in some scenarios and limitations. It results from specific design or implementation choices for traffic generation and TD detection. In this section, we will study these choices.

\subsection{Traffic generation}
The design of preserving application data and its timing from the original application network trace in replay script is crucial for Wehe's tool. Sometimes, it hinders the TD detection, as explained in  Sec. \ref{subsec:td_org_replay}. This design choice limits the TD detection capability as the traffic shaping rate is not the same across different ISPs.

The Wehe detects the content-based TD. This requirement leads the Wehe to design the probing data transmission on port number 80. The replay script based on the original application trace, as it is, does not lead to expected traffic classification by ISPs in all cases if it uses port 80 as described in Sec. \ref{subsec:port_80}. 

The Wehe designed the probing traffic as the traffic stream with original application data and traffic streams with a bit-reversed version of the same application data. It tends to provide unreliable throughput performances for comparison to detect TD, as explained in Sec. \ref{subsec:tr_load}.    

\subsection{TD detection}
Wehe's direct performance comparison design needs that performances of probing traffic are only affected by network policies. The use of exact application data and its timings from the original application provides this provision as its side effect of not exhausting the entire available bandwidth under a specific scenario. Another design choice of back-to-back replays tries to ensure it by making Wehe require minimum bandwidth to exchange probing traffic. Nevertheless, it adds more uncorrelated perturbations in the probing traffic performances under heavy time-varying load at the user-client side. 
The provision required for direct performance comparison is not guaranteed in specific traffic load scenarios, as explained in Sec. \ref{subsec:non_exhaust_bw} and disturbed by back-to-back replay design. 

The non-consideration of total network load at the user-client side in the Wehe tool design and back-to-back replay design makes the Wehe tool detect the TD due to background traffic load on the probing traffic performances. 

\subsection{Operation environment}
The Wehe implements the side-channel design to tackle various issues due to intermediate network devices, such as proxies or NAT devices. Nevertheless, it complicates the HTTP protocol based client-server communication and makes it non-manageable in the long run.

==> wehe__Manjesh_Kumar_Hanawal_s_conflicted_copy_2021-10-02_.tex <==
The Wehe \cite{wehe} is a tool for the detection of traffic differentiation over mobile networks (e.g., cellular and WiFi). It is available as an App on Android and the iOS platforms. The user database of the Wehe tool consists of 126,249 users across 2,735 ISPs in 183 countries/regions generating 1,045,413 crowd-sourced measurements. European national telecom regulator, the US FTC and FCC, US Senators, and numerous US state legislators have used the Wehe tool's findings. 

The tool supports TD detection for many popular services such as Netflix and YouTube. The tool runs TD detection tests by coordinating with its server, called the `replay server'. The replay server keeps track of active user-clients and maps replay runs to correct user's service. In the following we discuss  probe traffic generation, network responses and other operational requirements of Wehe.

\subsection{Traffic generation}
Wehe uses the ``record-and-replay" method for generating probing traffic. The user-client exchanges the probing traffic with the replay server as per the replay script that captures the application-level traffic behavior, including the port number, data sequence, and timing dependencies from original service's network logs. Preserving timing is a crucial feature of Wehe's approach. It expects network devices to use this information in case of non-availability of any other means to classify applications, e.g., HTTPS encrypted data transfer. 

Wehe uses two types of probing traffic streams. While one stream (\textit{original} replay) is same as the original services' application-level network trace, another traffic stream (\textit{control} replay) differs substantially from the first traffic stream. We uses uses two types of control traffic. In one type it uses the meddle VPN \cite{meddle} framework for data transfer and server-side packet capture. Another approach uses a bit-reversed version of the first traffic stream sent one the same channel. Currently, the Wehe uses the latter approach due to its superior results. 

\subsection{Over the network response}
Wehe is a differential detector tool that compares the network responses for two types of traffic streams generated by the tool. The service-specific information present in the \textit{original} replay is useful for network devices with Deep Packet Inspection (DPI) capability to identify and classify the service correctly. So, the \textit{original} replay's traffic performance over the Internet closely resembles the original application traffic on the same network. While \textit{original} replay is exposed for detection to network devices, the traffic streams with bit reversed data or \textit{control} replay is  `not detectable' for classification. Thus it is expected that the \textit{control} replay traffic evades the content-based application-specific traffic differentiation. The performances of two such traffic streams (detectable and non-detectable) differ if network devices apply different traffic management or traffic differentiation on each traffic stream as per content-based classification. 
%This differentiation is assumed to be triggered by many factors, such as IP addresses or port numbers. However, the Wehe App detects content-based traffic differentiation. It is evident from usage of specially crafted detectable \textit{original} replay that allows TD and non-detectable \textit{control} replay that evades TD.      
   
\subsection{TD detection scenario expectations}
Wehe compares the throughput performances of \textit{original} replay and \textit{control} replay to detect TD. The methodology uses the throughput as a comparison metric due to its sensitivity to bandwidth-limiting traffic shaping. However, the tool expects that the TD detection algorithm does not detect TD based on throughput for traffic streams with traffic rates below the shaping rate. The rationale is that the shaper cannot affect the performance of such an application stream. 

Many times both traffic streams get affected by other factors such as signal strength and congestion. It creates an irregularity in the received performance due to bandwidth volatility. It is mentioned to be leading to incorrect differentiation detection. The tool performs multiple test replays to overcome the effect of bandwidth volatility. 

\subsection{Operational requirements}
The Wehe server needs side-channels for each client to associate it with precisely one app replay. This side-channel supplies information about replay runs to the server. Each user directly connected to Wehe replay server is uniquely identifiable on the server-side with an associated IP address of side channels that maps each replay to exactly one App. 

The other operational requirement is that Wehe client-server communication uses customized socket connections with specific keep-alive behavior. Sometimes, the usage of translucent proxies by user-client modifies this behavior. The Replay server handles this situation by handling such unexpected connections. The protocol-specific proxies, e.g., HTTP proxy, connect the user-client to the server through itself using specific port numbers, e.g., 80/443 for HTTP/HTTPS. Nevertheless, it allows the user-client to connect to the server for connections using other protocols directly. The side-channels of Wehe does not use HTTP/HTTPS connection. So the IP address for the same user differs for side-channel and replay runs. Wehe server detects such connections and indicates such connections to the user-client using a special message. The special message triggers the exchange of further communication with a customized header. 

\subsection{Challenges of validating Wehe}
The Wehe tool is straightforward to use TD detection tool — the requirement changes when using it for its validation. The validation process may need to launch only one type of replay for different services during one test or may need to launch all replays in parallel. These are not requirements related to TD detection, Wehe's primary goal, so understandably not supported. Hence the validation of Wehe's working in such scenarios needs a specific client-server setup. Here the challenge is to separate the intended scenario-specific Wehe's mechanism so that the resulting system still mimics Wehe's actual behavior. 

Moreover, Wehe does not provide error/failure notifications in all scenarios. Instead, it prompts the user to reopen the App. As a result, the validation setup loses the vital feedback information regarding the error/failure induced by its validation scenario.
